The enhanced X-ray Timing and Polarimetry mission - eXTP

In this paper we present the enhanced X-ray Timing and Polarimetry mission - eXTP. eXTP is a space science mission designed to study fundamental physics under extreme conditions of density, gravity and magnetism. The mission aims at determining the equation of state of matter at supra-nuclear density, measuring effects of QED, and understanding the dynamics of matter in strong-field gravity. In addition to investigating fundamental physics, eXTP will be a very powerful observatory for astrophysics that will provide observations of unprecedented quality on a variety of galactic and extragalactic objects. In particular, its wide field monitoring capabilities will be highly instrumental to detect the electro-magnetic counterparts of gravitational wave sources. The paper provides a detailed description of: (1) the technological and technical aspects, and the expected performance of the instruments of the scientific payload; (2) the elements and functions of the mission, from the spacecraft to the ground segment.

==> dotar <==
tar cvf eXTP_WP_OS.tar \
2017SCGE.cls                    \
BB_1mCrab_ld_del_eemo_jz.eps	\
Clump.eps			\
collision.eps			\
dotar				\
elavsky4.png			\
eXTP_CV_fig.eps			\
extp.eps			\
eXTP_WP_OS.tex		\
facilities_vs9jan2018.pdf	\
famps_extp7.eps			\
figgrb1_vs6.eps			\
figgrb2b.pdf			\
figgrb3_vs3.eps			\
figgrbiron1_vs2.eps		\
figgrbiron2_vs2.eps		\
FoV_vs26092017.pdf		\
jean4m2.pdf			\
lc_extp5.eps			\
lmxb_orbitsn.pdf		\
LOFT_AGN_var_totcounts.pdf	\
patruno.png			\
radiomap3.eps			\
sens.pdf			\
snr1.eps			\
spectra.eps			\
stellarflare_artist.eps		\
v0332_crit.pdf                  \
wu2010.png                      \
picins.sty                      \
Print-CrossMark.eps                  \
Print-CrossMark-eps-converted-to.pdf \
figDrake3b.eps                       \
sn1006_1_srcut_sfa_1e4.eps           \
eXTP_WP_OS.pdf

gzip eXTP_WP_OS.tar

